Constriction of actin rings by passive crosslinkers

In many organisms, cell division is driven by the constriction of a cytokinetic ring, which consists of actin filaments and crosslinking proteins. While it has long been believed that the constriction is driven by motor proteins, it has recently been discovered that passive crosslinkers that do not turn over fuel are able to generate enough force to constrict actin filament rings. To study the ring constriction dynamics, we develop a model that includes the driving force of crosslinker condensation and the opposing forces of friction and filament bending. We analyze the constriction force as a function of ring topology and crosslinker concentration, and predict forces that are sufficient to constrict an unadorned plasma membrane. Our model also predicts that actin-filament sliding arises from an interplay between filament rotation and crosslinker hopping, producing frictional forces that are low compared to those of crosslinker-mediated microtubule sliding.

==> tex/glossary.tex <==
% glossary.tex

\begin{acronym}
    \acro{FEM}{finite element method}
    \acro{MC}{Monte Carlo}
    \acro{PDE}{partial differential equation}
    \acro{US}{umbrella sampling}
    \acro{WLC}{worm-like chain}
\end{acronym}


==> tex/macros.tex <==
% macros.tex

\makeatletter
\newcommand{\defaultcolor}[1]{%
  \color{#1}\global\let\default@color\current@color
}
\makeatother

\newcommand\supplemental{%
    \xdef\presupfigures{\arabic{figure}}% save the current figure number
    \xdef\presupsections{\arabic{section}}% save the current section number
    \xdef\presupequations{\arabic{equation}}% save the current section number
    \xdef\presuptables{\arabic{table}}% save the current section number
    \renewcommand\thefigure{S\fpeval{\arabic{figure}-\presupfigures}}
    \renewcommand\thesection{S\fpeval{\arabic{section}-\presupsections}}
    \renewcommand\theequation{S\fpeval{\arabic{equation}-\presupequations}}
    \renewcommand\thetable{S\fpeval{\arabic{table}-\presuptables}}
}

% Redefine \maketitle so that it can be used twice (for supplementary)
\makeatletter
\def\maketitle{
\@author@finish
\title@column\titleblock@produce
\suppressfloats[t]}
\makeatother

\renewcommand{\binom}[2]{\mleft(\genfrac{}{}{0pt}{}{#1}{#2}\mright)}

% Equilibrium radius
\newcommand{\Req}{R_\mathrm{eq}}
\newcommand{\Rmax}{R_\mathrm{max}}
\newcommand{\Rmin}{R_\mathrm{min}}

% Derivative
\newcommand{\deriv}[2]{\frac{\mathrm{d} #1}{\mathrm{d} #2}}

% Partial derivative
\newcommand{\pderiv}[2]{\frac{\partial #1}{\partial #2}}

% Exponential
\newcommand{\expsup}[1]{\mathrm{e}^{#1}}

% Boltzmann's constant
\newcommand{\kb}{k_{\mathrm{B}}}

% Dissociation constant for pair binding
\newcommand{\Kd}{K_\mathrm{D}^\mathrm{d}}

% Dissociation constant for single binding
\newcommand{\Ks}{K_\mathrm{D}^\mathrm{s}}

% Total number of filaments
\newcommand{\Nf}{N_\mathrm{f}}

% Number of scaffold filaments
\newcommand{\Nsca}{N_\mathrm{sca}}

% Number of overlaps
\newcommand{\No}{N_\mathrm{o}}

% Number of doubly bound crosslinkers
\newcommand{\Nd}{N_\mathrm{d}}

% Total number of doubly bound crosslinkers
\newcommand{\Ndtot}{N_\text{d, tot}}

% Number of doubly bound crosslinkers of overlap i
\newcommand{\Ndi}{N_\text{d, i}}

% Number of singly bound crosslinkers
\newcommand{\Ns}{N_\mathrm{s}}

% Number of singly bound sites
\newcommand{\Nss}{N_\mathrm{ss}}

% Number of doubly singly bound sites
\newcommand{\Nb}{N_\mathrm{b}}

% Number of right-pulling crosslinkers
\newcommand{\NR}{N_\mathrm{R}}

% Length of filament
\newcommand{\Lf}{L_\mathrm{f}}

% Total number of overlap sites
\newcommand{\Ltot}{L_\mathrm{tot}}

% Total number of overlap sites
\newcommand{\ltot}{\ell_\mathrm{tot}}

% Diameter of filament
\newcommand{\Df}{\diameter_\mathrm{f}}

% Sites per filament
\newcommand{\lf}{l_\mathrm{f}}

% Filament diffusion constant
\newcommand{\DLf}{D_\mathrm{f}}

% Rates
\newcommand{\rzo}{r_\text{0, 1}}
\newcommand{\rzt}{r_\text{0, 2}}
\newcommand{\rot}{r_\text{1, 2}}
\newcommand{\rto}{r_\text{2, 1}}
\newcommand{\roz}{r_\text{1, 0}}
\newcommand{\rtz}{r_\text{2, 0}}

\newcommand{\deltas}{\delta_\mathrm{s}}
\newcommand{\deltad}{\delta_\mathrm{d}}
\newcommand{\rhod}{\rho_\mathrm{d}}
\newcommand{\rhos}{\rho_\mathrm{s}}

\newcommand{\zetaf}{\zeta_\mathrm{f}}
\newcommand{\zetaR}{\zeta_\mathrm{R}}
\newcommand{\ForceR}{F_\mathrm{R}}

\DeclareSIUnit\molar{M}

%\newcommand{\AMCcomment}[1]{\todo[size=\scriptsize,color=green!20]{[AMC]:#1}}
%\newcommand{\AMCcommenti}[1]{\todo[inline,size=\scriptsize,color=green!20]{[AMC]:#1}\noindent}

